PanSplat: 4K Panorama Synthesis with Feed-Forward Gaussian Splatting

With the advent of portable 360{\deg} cameras, panorama has gained significant attention in applications like virtual reality (VR), virtual tours, robotics, and autonomous driving. As a result, wide-baseline panorama view synthesis has emerged as a vital task, where high resolution, fast inference, and memory efficiency are essential. Nevertheless, existing methods are typically constrained to lower resolutions (512 $\times$ 1024) due to demanding memory and computational requirements. In this paper, we present PanSplat, a generalizable, feed-forward approach that efficiently supports resolution up to 4K (2048 $\times$ 4096). Our approach features a tailored spherical 3D Gaussian pyramid with a Fibonacci lattice arrangement, enhancing image quality while reducing information redundancy. To accommodate the demands of high resolution, we propose a pipeline that integrates a hierarchical spherical cost volume and Gaussian heads with local operations, enabling two-step deferred backpropagation for memory-efficient training on a single A100 GPU. Experiments demonstrate that PanSplat achieves state-of-the-art results with superior efficiency and image quality across both synthetic and real-world datasets. Code is available at https://github.com/chengzhag/PanSplat.

==> figure/cmp_2row.tex <==
{
\newcommand{\cmptworow}[1]{
    \begin{figure*}[t]
        % \vspace{-2em}
        \centering
        \small
        \setlength\tabcolsep{1px}
        \resizebox{1.\linewidth}{!}{
            \begin{tabular}{rccccc}
                #1
                & Input/GT Views & PanoGRF & MVSplat & PanSplat & GT Crop
            \end{tabular}
        }
        % \vspace{-0.5em}
        \caption{
            Qualitative comparison among PanoGRF, MVSPlat and PanSplat.
        }
        % \vspace{-0.5em}
    \end{figure*}
}

\newcommand{\row}[4]{
    \rotatebox[origin=c]{90}{
        \makecell[c]{
            \newcolumntype{C}[1]{>{\hsize=##1\hsize\centering\arraybackslash}X}
            \begin{tabularx}{0.32\linewidth}{C{0.66}C{0.66}C{0.66}}
                Input View 2 & GT View & Input View 1
            \end{tabularx}
        }
    } &
    \makecell[c]{
        \includegraphics[width=0.209\linewidth]{results/#1/in_0/#2.jpg}
        \\
        \includegraphics[width=0.209\linewidth]{results/#1/gt/#2.jpg}
        \\
        \includegraphics[width=0.209\linewidth]{results/#1/in_1/#2.jpg}
    } &
    \makecell{
        \includegraphics[width=0.16\linewidth, clip, trim={#3}]{results/#1/panogrf/#2.jpg}
        \\
        \includegraphics[width=0.16\linewidth, clip, trim={#4}]{results/#1/panogrf/#2.jpg}
    } &
    \makecell{
        \includegraphics[width=0.16\linewidth, clip, trim={#3}]{results/#1/mvsplat/#2.jpg}
        \\
        \includegraphics[width=0.16\linewidth, clip, trim={#4}]{results/#1/mvsplat/#2.jpg}
    } &
    \makecell{
        \includegraphics[width=0.16\linewidth, clip, trim={#3}]{results/#1/pansplat/#2.jpg}
        \\
        \includegraphics[width=0.16\linewidth, clip, trim={#4}]{results/#1/pansplat/#2.jpg}
    } &
    \makecell{
        \includegraphics[width=0.16\linewidth, clip, trim={#3}]{results/#1/gt/#2.jpg}
        \\
        \includegraphics[width=0.16\linewidth, clip, trim={#4}]{results/#1/gt/#2.jpg}
    }
    \\
}

\cmptworow{
    \row{cmp_mp3d}{0}{239px 190px 593px 130px}{0px 25px 884px 347px}
    \row{cmp_mp3d}{5}{184px 50px 700px 322px}{559px 150px 273px 170px}
}
\cmptworow{
    \row{cmp_replica}{17}{79px 160px 753px 160px}{700px 185px 184px 187px}
    \row{cmp_replica}{8}{0px 20px 884px 352px}{629px 150px 243px 210px}
}
\cmptworow{
    \row{cmp_residential}{1}{872px 170px 0px 190px}{610px 235px 274px 137px}
    \row{cmp_residential}{2}{400px 120px 484px 252px}{270px 130px 634px 262px}
}
}

==> figure/cmp_mp3d.tex <==
{
\newcommand{\resultsfigwidth}{1.5in}
\newcommand{\resultscropwidth}{0.75in}
% \renewcommand{\resultscropwidth}{0.79in}
% Define the crops here, individually for each image
\newcommand{\cropcmpfirst}[1]{
  \makecell{
  % left bottom right top
  % {"bbox": [218, 211, 584, 79]}
  \includegraphics[trim={218px 211px  584px 79px}, clip, width=\resultscropwidth]{#1} \\
  % {"bbox": [4, 2, 845, 335]}
  \includegraphics[trim={4px 2px 845px 335px}, clip, width=\resultscropwidth]{#1} 
  }
}
\newcommand{\cropcmpsecond}[1]{
  \makecell{
  % left bottom right top
% {"bbox": [663, 100, 250, 301]}
  \includegraphics[trim={663px 110px  250px 301px}, clip, width=\resultscropwidth]{#1} \\
  % {"bbox": [4, 2, 845, 335]}
  % {"bbox": [154, 83, 787, 346]}
  \includegraphics[trim={154px 83px 787px 346px}, clip, width=\resultscropwidth]{#1} 
  }
}
\newcommand{\cropcmpthird}[1]{
  \makecell{
  % left bottom right top
\includegraphics[trim={115px 108px 703px 198px}, clip, width=\resultscropwidth]{#1} \\
% {"bbox": [321, 22, 540, 327]}
  \includegraphics[trim={321px 22px 540px 327px}, clip, width=\resultscropwidth]{#1} 
  }
}
\newcommand{\cropcmpforth}[1]{
  \makecell{
  % left bottom right top
  % {"bbox": [111, 149, 844, 294]}
\includegraphics[trim={111px 149px 844px 294px}, clip, width=\resultscropwidth]{#1} \\
  \includegraphics[trim={375px 4px 426px 285px}, clip, width=\resultscropwidth]{#1} 
  }
}
\newcommand{\cropcmpfifth}[1]{
  \makecell{
  % left bottom right top
  % {"bbox": [111, 149, 844, 294]}
  % {"bbox": [247, 72, 571, 234]}
\includegraphics[trim={247px 72px 571px 234px}, clip, width=\resultscropwidth]{#1} \\
% {"bbox": [636, 1, 203, 326]}
  \includegraphics[trim={636px 1px 203px 326px}, clip, width=\resultscropwidth]{#1} 
  }
}

\newcommand{\cropcmpsixth}[1]{
  \makecell{
  % left bottom right top
  % {"bbox": [218, 211, 584, 79]}
  % {"bbox": [349, 19, 392, 210]}
  \includegraphics[trim={349px 19px  392px 210px}, clip, width=\resultscropwidth]{#1} 
  \\
  \includegraphics[trim={541px 308px 289px 10px}, clip, width=\resultscropwidth]{#1} 
  }
}
\newcommand{\cropcmpmt}[1]{
  \makecell{
  % left bottom right top
  % {"bbox": [218, 211, 584, 79]}
  % {"bbox": [349, 19, 392, 210]}
  \includegraphics[trim={84px 75px  800px 297px}, clip, width=\resultscropwidth]{#1} 
  \\
  \includegraphics[trim={489px 80px 243px 140px}, clip, width=\resultscropwidth]{#1} 
  }
}


% % {"bbox": [89, 95, 830, 312]}
% \newcommand{\cropcmpmatterport}[1]{
%   \makecell{
%   % left bottom right top
%   % {"bbox": [84, 75, 800, 297]}
%   \includegraphics[trim={84px 75px  800px 297px}, clip, width=\resultscropwidth]{#1}
  
%   \\
%   % {"bbox": [489, 80, 243, 140]}
%   \includegraphics[trim={489px 80px 243px 140px}, clip, width=\resultscropwidth]{#1} 
%   }
% }


% \newcommand{\resultsfigwidth}{1.5in}
% \newcommand{\resultscropwidth}{0.7in}
% \renewcommand{\resultscropwidth}{0.79in}
% Define the crops here, individually for each image

\begin{figure*}[htbp]
\vspace{-10pt}
\centering
\scriptsize
\begin{tabular}{@{}c@{\,\,}c@{}c@{}c@{}c@{}c@{}c@{}c@{}c@{}c@{}}
\setlength{\tabcolsep}{10pt}
% \begin{tabular}{@{}c@{\,\,}c@{\,\,}c@{}c@{}c@{}c@{}}
% \begin{tabular}{ccccc}
% \makecell[c]{
% \includegraphics[trim={0px 0px 0px 0px}, clip, width=\resultsfigwidth]{results/cmp_mp3d/gt_draw/0.jpg}
% \\
% \textit{Sample 1}
% }
% & 
% \cropcmpfirst{results/cmp_mp3d/gt/0.jpg} &
% \cropcmpfirst{results/cmp_mp3d/ibrnet/0.jpg} &
% \cropcmpfirst{results/cmp_mp3d/omnisyn/0.jpg} &
% \cropcmpfirst{results/cmp_mp3d/neuray/0.jpg} &
% \cropcmpfirst{results/cmp_mp3d/panogrf/0.jpg}

% \\
% \makecell[c]{
% \includegraphics[trim={0px 0px 0px 0px}, clip, width=\resultsfigwidth]{results/cmp_mp3d/gt_draw/1.jpg}
% \\
% \textit{Sample 2}
% }
% & 
% \cropcmpsecond{results/cmp_mp3d/gt/1.jpg} &
% \cropcmpsecond{results/cmp_mp3d/ibrnet/1.jpg} &
% \cropcmpsecond{results/cmp_mp3d/omnisyn/1.jpg} &
% \cropcmpsecond{results/cmp_mp3d/neuray/1.jpg} &
% \cropcmpsecond{results/cmp_mp3d/panogrf/1.jpg}
% \\
% \makecell[c]{
% \includegraphics[trim={0px 0px 0px 0px}, clip, width=\resultsfigwidth]{results/cmp_replica/gt_draw/1.jpg}
% \\
% \textit{Sample 3}
% }
% & 
% \cropcmpthird{results/cmp_replica/gt/1.jpg} &
% \cropcmpthird{results/cmp_replica/ibrnet/1.jpg} &
% \cropcmpthird{results/cmp_replica/omnisyn/1.jpg} &
% \cropcmpthird{results/cmp_replica/neuray/1.jpg} &
% \cropcmpthird{results/cmp_replica/panogrf/1.jpg}
\\

\makecell[c]{
\includegraphics[trim={0px 0px 0px 0px}, clip, width=\resultsfigwidth]{results/cmp_replica/gt_draw/6.jpg}
\\
\textit{Sample 1 (Replica)}
}
&
\cropcmpfifth{results/cmp_replica/omnisyn/6.jpg} &
\cropcmpfifth{results/cmp_replica/ibrnet/6.jpg} &
\cropcmpfifth{results/cmp_replica/neuray/6.jpg} &
\cropcmpfifth{results/cmp_replica/panogrf/6.jpg} &
\cropcmpfifth{results/cmp_replica/mvsplat/6.jpg} &
\cropcmpfifth{results/cmp_replica/pansplat/6.jpg}
&
\cropcmpfifth{results/cmp_replica/gt/6.jpg}  
\\
\makecell[c]{
\includegraphics[trim={0px 0px 0px 0px}, clip, width=\resultsfigwidth]{results/cmp_mp3d/gt_draw/7.jpg}
\\
\textit{Sample 2 (Matterport3D)}
}
&

\cropcmpmt{results/cmp_mp3d/omnisyn/7.jpg} &
\cropcmpmt{results/cmp_mp3d/ibrnet/7.jpg} &
\cropcmpmt{results/cmp_mp3d/neuray/7.jpg} &
\cropcmpmt{results/cmp_mp3d/panogrf/7.jpg} &
\cropcmpmt{results/cmp_mp3d/mvsplat/7.jpg} &
\cropcmpmt{results/cmp_mp3d/pansplat/7.jpg}
&
\cropcmpmt{results/cmp_mp3d/gt/7.jpg}  
\\

& OmniSyn & IBRNet$^{*}$ & NeuRay$^{*}$ & PanoGRF & MVSplat & PanSplat & Ground Truth


% \\


% \makecell[c]{
% \includegraphics[trim={0px 0px 0px 0px}, clip, width=\resultsfigwidth]{results/cmp_residential/gt_draw/0.jpg}
% \\
% \textit{Sample 3 (Residential)}
% }
% & 
% \cropcmpsixth{results/cmp_residential/ibrnet/0.jpg} &
% \cropcmpsixth{results/cmp_residential/nerf/0.jpg} &
% \cropcmpsixth{results/cmp_residential/neuray/0.jpg} &
% \cropcmpsixth{results/cmp_residential/panogrf/0.jpg} &
% \cropcmpsixth{results/cmp_residential/gt/0.jpg} 

% \\

%  &IBRNet$^{*}$ & S-NeRF &NeuRay$^{*}$  & PanoGRF & Ground Truth

\end{tabular}
\caption{
  Qualitative comparison on Replica and Matterport3D among OmniSyn, IBRNet$^*$, NeuRay$^*$, PanoGRF, MVSplat and PanSplat.
}
\vspace{-5pt}
\label{fig:res-cmp}
\end{figure*}
}

==> figure/cmp_residential.tex <==
{
\newcommand{\resultsfigwidth}{1.5in}
\newcommand{\resultscropwidth}{0.75in}
% \renewcommand{\resultscropwidth}{0.79in}
% Define the crops here, individually for each image
\newcommand{\cropcmpfirstres}[1]{
  \makecell{
  % left bottom right top
  % {"bbox": [218, 211, 584, 79]}
  % {"bbox": [349, 19, 392, 210]}
  \includegraphics[trim={349px 19px  392px 210px}, clip, width=\resultscropwidth]{#1} 
  \\
  \includegraphics[trim={541px 308px 289px 10px}, clip, width=\resultscropwidth]{#1} 
  }
}

% % {"bbox": [89, 95, 830, 312]}
% \newcommand{\cropcmpsecondres}[1]{
%   \makecell{
%   \includegraphics[trim={393px 80px  374px 175px}, clip, width=\resultscropwidth]{#1} 
%   \\
%   \includegraphics[trim={885px 232px 1px 142px}, clip, width=\resultscropwidth]{#1} 
%   }
% }
\newcommand{\cropcmpsecondres}[1]{
  \makecell{
  % left bottom right top
  % {"bbox": [218, 211, 584, 79]}
  % {"bbox": [349, 19, 392, 210]}
  \includegraphics[trim={393px 80px  374px 175px}, clip, width=\resultscropwidth]{#1} 
  \\
  \includegraphics[trim={885px 232px 1px 142px}, clip, width=\resultscropwidth]{#1} 
  }
}
 
\begin{figure*}[htbp]
% \vspace{-5pt}
\centering
\scriptsize
\begin{tabular}{@{}c@{\,\,}c@{}c@{}c@{}c@{}c@{}c@{}c@{}}
\setlength{\tabcolsep}{10pt}
% \begin{tabular}{@{}c@{\,\,}c@{\,\,}c@{}c@{}c@{}c@{}}
% \begin{tabular}{ccccc}

 \\
 \makecell[c]{
\includegraphics[trim={0px 0px 0px 0px}, clip, width=\resultsfigwidth]{results/cmp_residential/gt_draw/0.jpg}
\\
\textit{Sample 1 (Residential)}
}
 &
\cropcmpfirstres{results/cmp_residential/nerf/0.jpg} &
\cropcmpfirstres{results/cmp_residential/ibrnet/0.jpg} &
\cropcmpfirstres{results/cmp_residential/neuray/0.jpg} &
\cropcmpfirstres{results/cmp_residential/panogrf/0.jpg} &
\cropcmpfirstres{results/cmp_residential/mvsplat/0.jpg} &
\cropcmpfirstres{results/cmp_residential/pansplat/0.jpg}
&
\cropcmpfirstres{results/cmp_residential/gt/0.jpg}
\\
% \cropcmpsecondres{results/cmp_residential/nerf/0.jpg} &
% \cropcmpfirstres{results/cmp_residential/ibrnet/0.jpg} &
% \cropcmpfirstres{results/cmp_residential/neuray/0.jpg} &
% \cropcmpfirstres{results/cmp_residential/panogrf/0.jpg}& 
% \cropcmpfirstres{results/cmp_residential/gt/0.jpg} &
% \makecell[c]{
% \includegraphics[trim={0px 0px 0px 0px}, clip, width=\resultsfigwidth]{results/cmp_residential/gt_draw/0.jpg}
% \\
% \textit{Residential}
% }
\makecell[c]{
\includegraphics[trim={0px 0px 0px 0px}, clip, width=\resultsfigwidth]{results/cmp_residential/gt_draw/1.jpg}
\\
\textit{Sample 2 (Residential)}
}

  &
\cropcmpsecondres{results/cmp_residential/nerf/1.jpg} &
\cropcmpsecondres{results/cmp_residential/ibrnet/1.jpg} &
\cropcmpsecondres{results/cmp_residential/neuray/1.jpg} &
\cropcmpsecondres{results/cmp_residential/panogrf/1.jpg} &
\cropcmpsecondres{results/cmp_residential/mvsplat/1.jpg} &
\cropcmpsecondres{results/cmp_residential/pansplat/1.jpg}
&
\cropcmpsecondres{results/cmp_residential/gt/1.jpg}
\\
 &
 S-NeRF  &IBRNet$^{*}$ &NeuRay$^{*}$  & PanoGRF & MVSplat & PanSplat & Ground Truth
\end{tabular}
\caption{
  Qualitative comparison on Residential between S-NeRF, IBRNet$^*$, NeuRay$^*$, PanoGRF, MVSplat and PanSplat.
}
\vspace{-5pt}
\label{fig:cmp_residential}
\end{figure*}
}

==> figure/frame_dis_fig.tex <==
{

\newcommand{\row}[4]{
    \raisebox{10ex}{\rotatebox[origin=c]{90}{#1}} &
    \includegraphics[width=0.19\linewidth, clip, trim={#4}]{results/cmp_insta360/#2/#3/0.jpg} &
    \includegraphics[width=0.19\linewidth, clip, trim={#4}]{results/cmp_insta360/#2/#3/4.jpg} &
    \includegraphics[width=0.19\linewidth, clip, trim={#4}]{results/cmp_insta360/#2/#3/8.jpg} &
    \includegraphics[width=0.19\linewidth, clip, trim={#4}]{results/cmp_insta360/#2/#3/12.jpg} &
    \includegraphics[width=0.19\linewidth, clip, trim={#4}]{results/cmp_insta360/#2/#3/16.jpg}
    \\
}

\newcommand{\cmpframes}[2]{
    \centering
    \scriptsize
    \setlength\tabcolsep{1px}
    \resizebox{1.\linewidth}{!}{
        \begin{tabular}{rccccc}
            \row{PanSplat}{pansplat}{#1}{#2}
            \row{+ Deferred BL}{pansplat_defbl}{#1}{#2}
            & Frame \#0 & Frame \#4 & Frame \#8 & Frame \#12 & Frame \#16
        \end{tabular}
    }
}

\begin{figure*}[t]
    \centering
    \begin{subfigure}[c]{0.3\textwidth}
        \centering
        \includegraphics[width=\linewidth, trim={710px 0 0 0}, clip]{figure/frame_vs_metric.pdf}
        % \caption{Metric Plot}
    \end{subfigure}
    \hspace{0.01\textwidth} % Space between subfigures
    \begin{subfigure}[c]{0.68\textwidth}
        \centering
        % \cmpframes{VID_20240914_103257_00_005-008839_008855}{703px 140px 119px 170px}
        \cmpframes{VID_20240914_103257_00_005-009712_009728}{109px 15px 433px 15px}
        % \cmpframes{VID_20240922_102141_00_006-003972_003988}{509px 15px 133px 115px}
        % \cmpframes{VID_20240922_102141_00_006-005959_005975}{409px 15px 333px 215px}
        % \caption{Comparison Frames}
    \end{subfigure}
    \vspace{-0.5em}
    \caption{
        Comparison on different frame distances.
    }\label{fig:frame_dis}
    % \vspace{-1em}
\end{figure*}

}


==> table/cmp_mp3d.tex <==
\begin{table*}[t]
    \setlength\tabcolsep{2pt}
    \centering
    \begin{tabular}{cccccccccc}
        \toprule
        Baseline & \multicolumn{3}{c}{1.0m} & \multicolumn{3}{c}{1.5m} & \multicolumn{3}{c}{2.0m} \\
        \cmidrule(lr){1-1}\cmidrule(lr){2-4}\cmidrule(lr){5-7}\cmidrule(lr){8-10}
        Method & WS-PSNR$\uparrow$ & SSIM$\uparrow$ & LPIPS$\downarrow$ & WS-PSNR$\uparrow$ & SSIM$\uparrow$ & LPIPS$\downarrow$ & WS-PSNR$\uparrow$ & SSIM$\uparrow$ & LPIPS$\downarrow$\\
        \cmidrule(lr){1-1}\cmidrule(lr){2-4}\cmidrule(lr){5-7}\cmidrule(lr){8-10}
        S-NeRF  & 15.25 & 0.579 & 0.546 & 14.16 & 0.563 & 0.580 & 13.13 & 0.523 & 0.607 \\
        OmniSyn & 22.90 & 0.850 & 0.244 & 20.31 & 0.790 & 0.317 & 18.91 & \cellcolor{orange!30}0.761 & \cellcolor{yellow!30}0.354 \\
        IBRNet  & 25.72 & 0.855 & 0.258 & 21.69 & 0.751 & 0.382 & \cellcolor{yellow!30}20.04 & 0.706 & 0.431 \\
        NeuRay & 24.92 & 0.832 & 0.260 & 21.92 & 0.766 & 0.347 & 19.85 & \cellcolor{yellow!30}0.715 & 0.407 \\
        PanoGRF & \cellcolor{yellow!30}27.12 & \cellcolor{yellow!30}0.876 & \cellcolor{yellow!30}0.195 & \cellcolor{orange!30}23.38 & \cellcolor{orange!30}0.811 & \cellcolor{yellow!30}0.282 & \cellcolor{orange!30}20.96 & \cellcolor{orange!30}0.761 & \cellcolor{orange!30}0.352 \\
        MVSplat & \cellcolor{orange!30}29.29 & \cellcolor{orange!30}0.912 & \cellcolor{orange!30}0.105 & \cellcolor{yellow!30}22.51 & \cellcolor{yellow!30}0.807 & \cellcolor{orange!30}0.230 & 13.38 & 0.595 & 0.554 \\ % qbn2ltku
        PanSplat & \cellcolor{red!30}30.01 & \cellcolor{red!30}0.931 & \cellcolor{red!30}0.091 & \cellcolor{red!30}24.76 & \cellcolor{red!30}0.849 & \cellcolor{red!30}0.181 & \cellcolor{red!30}21.19 & \cellcolor{red!30}0.777 & \cellcolor{red!30}0.265 \\ % nvpl49ge
        \bottomrule
    \end{tabular}
    \vspace{-0.5em}
    \caption{
        Quantitative comparison on Matterport3D.
        The best, second, third results are highlighted in \textcolor{red}{red}, \textcolor{orange}{orange}, and \textcolor{yellow}{yellow}, respectively.
    }\label{tbl:cmp_mp3d}
\end{table*}


==> table/cmp_replica.tex <==
\begin{table*}[t]
    \setlength\tabcolsep{4pt}
    \centering
    \begin{tabular}{ccccccccc}
        \toprule
        Dataset & \multicolumn{4}{c}{Replica (1.0m baseline)}&\multicolumn{4}{c}{Residential (about 0.3m baseline)}\\
        \cmidrule(r){1-1}    \cmidrule(r){2-5} \cmidrule(r){6-9}
        Method & PSNR$\uparrow$ & WS-PSNR$\uparrow$ & SSIM$\uparrow$ & LPIPS$\downarrow$ & PSNR$\uparrow$ & WS-PSNR$\uparrow$ & SSIM$\uparrow$ & LPIPS$\downarrow$\\
        % \midrule
        \cmidrule(r){1-1}    \cmidrule(r){2-5} \cmidrule(r){6-9}
        S-NeRF & 16.91 & 16.10 &0.723 & 0.443& 23.06 & 22.47 & 0.741 & 0.435\\
        OmniSyn & 23.91 & 23.17 & 0.898&0.189&-&-&-&-\\
        IBRNet & 23.35 & 22.65 & 0.854 &0.291& 22.95 & 22.47 & 0.735 &0.498 \\
        NeuRay & 26.62 & 25.90 & 0.899 &0.187 & 23.01 & 22.38 & 0.753 &0.427\\
        PanoGRF & \cellcolor{yellow!30}30.08 & \cellcolor{yellow!30}29.22 & \cellcolor{yellow!30}0.937 & \cellcolor{yellow!30}0.134 & \cellcolor{red!30}31.64 & \cellcolor{yellow!30}31.03 & \cellcolor{orange!30}0.909 & \cellcolor{yellow!30}0.207\\
        MVSplat & \cellcolor{orange!30}31.25 & \cellcolor{orange!30}31.25 & \cellcolor{orange!30}0.958 & \cellcolor{red!30}0.059 & \cellcolor{yellow!30}31.32 & \cellcolor{orange!30}31.32 & \cellcolor{yellow!30}0.906 & \cellcolor{orange!30}0.200 \\ % qbn2ltku
        PanSplat & \cellcolor{red!30}31.68 & \cellcolor{red!30}31.67 & \cellcolor{red!30}0.962 & \cellcolor{orange!30}0.069 & \cellcolor{orange!30}31.42 & \cellcolor{red!30}31.36 & \cellcolor{red!30}0.917 & \cellcolor{red!30}0.172 \\ % nvpl49ge      
        \bottomrule
    \end{tabular}
    \vspace{-0.5em}
    \caption{
        Quantitative comparison on Replica and Residential.
    }\label{tbl:cmp_replica}
\end{table*}
